Default Disambiguation for Online Parsers

Since composed grammars are often ambiguous, grammar composition requires a mechanism for dealing with ambiguity: either ruling it out by using delimiters (which are awkward to work with), or by using disambiguation operators to filter a parse forest down to a single parse tree (where, in general, we cannot be sure that we have covered all possible parse forests). In this paper, we show that default disambiguation, which is inappropriate for batch parsing, works well for online parsing, where it can be overridden by the user if necessary. We extend language boxes -- a delimiter-based algorithm atop incremental parsing -- in such a way that default disambiguation can automatically insert, remove, or resize, language boxes, leading to the automatic language boxes algorithm. The nature of the problem means that default disambiguation cannot always match a user's intention. However, our experimental evaluation shows that automatic language boxes behave acceptably in 98.8% of tests involving compositions of real-world programming languages.

==> Makefile <==
.SUFFIXES: .tex .ps .dia .pdf .svg

.dia.pdf:
	dia -e eps-builtin -n -e ${@:.pdf=.eps} $<
	ps2pdf -dEPSCrop ${@:.pdf=.eps} $@

.svg.pdf:
	inkscape --export-pdf=$@ $<

LATEX_FILES = auto_lbox.tex

DIAGRAMS = images/limitation_php.pdf \
		   images/autoremoval.pdf \
		   images/sampleparsetree.pdf \
		   images/lbox_parsetree.pdf

EXTRA_DISTRIB_FILES = auto_lbox.pdf Makefile

all: auto_lbox.pdf

bib.bib: softdevbib/softdev.bib
	softdevbib/bin/prebib softdevbib/softdev.bib > bib.bib

softdevbib-update: softdevbib
	cd softdevbib && git pull

softdevbib/softdev.bib: softdevbib

softdevbib:
	git clone https://github.com/softdevteam/softdevbib.git


# Package up the paper for arxiv.org.
# Note that acmart.cls is included in tex live 2016, but it is too old.
ARXIV_FILES= softdev.sty \
		bib.bib \
		auto_lbox.bbl \

ARXIV_BASE=arxiv
${ARXIV_BASE}: auto_lbox.pdf acmart
	mkdir $@
	rsync -Rav ${ARXIV_FILES} $@
	cp auto_lbox.tex $@/auto_lbox.tex
	cp acmart.cls $@
	cp acmart/acmart.dtx $@
	cp acmart/acmart.ins $@
	zip -r $@.zip ${ARXIV_BASE}

ACMART_VERSION=904956ed0f4545da4fbb7f2401318917a348ba75
acmart:
	git clone https://github.com/borisveytsman/acmart
	cd acmart && git checkout ${ACMART_VERSION}

clean-arxiv:
	rm -rf arxiv
	rm -rf arxiv.zip
	rm -rf acmart

clean: clean-arxiv
	rm -rf ${DIAGRAMS} ${DIAGRAMS:S/.pdf/.eps/}
	rm -rf auto_lbox.aux auto_lbox.bbl auto_lbox.blg \
		auto_lbox.dvi auto_lbox.log auto_lbox.ps auto_lbox.pdf \
		auto_lbox.toc auto_lbox.out auto_lbox.snm auto_lbox.nav \
		auto_lbox.vrb texput.log bib.bib

auto_lbox.pdf: ${LATEX_FILES} ${DIAGRAMS} bib.bib
	pdflatex auto_lbox.tex
	bibtex auto_lbox
	pdflatex auto_lbox.tex
	pdflatex auto_lbox.tex

artefact.pdf: artefact.tex
	pdflatex artefact.tex
	pdflatex artefact.tex

